Error Feedback Reloaded: From Quadratic to Arithmetic Mean of Smoothness Constants

Error Feedback (EF) is a highly popular and immensely effective mechanism for fixing convergence issues which arise in distributed training methods (such as distributed GD or SGD) when these are enhanced with greedy communication compression techniques such as TopK. While EF was proposed almost a decade ago (Seide et al., 2014), and despite concentrated effort by the community to advance the theoretical understanding of this mechanism, there is still a lot to explore. In this work we study a modern form of error feedback called EF21 (Richtarik et al., 2021) which offers the currently best-known theoretical guarantees, under the weakest assumptions, and also works well in practice. In particular, while the theoretical communication complexity of EF21 depends on the quadratic mean of certain smoothness parameters, we improve this dependence to their arithmetic mean, which is always smaller, and can be substantially smaller, especially in heterogeneous data regimes. We take the reader on a journey of our discovery process. Starting with the idea of applying EF21 to an equivalent reformulation of the underlying problem which (unfortunately) requires (often impractical) machine cloning, we continue to the discovery of a new weighted version of EF21 which can (fortunately) be executed without any cloning, and finally circle back to an improved analysis of the original EF21 method. While this development applies to the simplest form of EF21, our approach naturally extends to more elaborate variants involving stochastic gradients and partial participation. Further, our technique improves the best-known theory of EF21 in the rare features regime (Richtarik et al., 2023). Finally, we validate our theoretical findings with suitable experiments.

==> experiments.tex <==
%\input{new_commands}
%\input{theorem_environments}
%\input{new_math_operators}
%\input{notes}

%\begin{document}	
%	\maketitle
%	\romantableofcontents
	
	\subsection{Characterization of Our Improvement}
	The standard \algname{EF21} analysis \cite{richtarik2021ef21} via Theorem 1 allows to perform the optimization procedure with maximum allowable step size $\gamma$ equal to:
	\begin{eqnarray}
		\label{frm:ef21_std}
		\gamma = \left( L + \tilde{L} \sqrt{\dfrac{\beta}{\theta}} \right)^{-1}, \theta = 1 - \sqrt{1-\alpha}, \beta=\dfrac{1-\alpha}{1 - \sqrt{1-\alpha}}
	\end{eqnarray}
	
	In Equation \ref{frm:ef21_std} the parameter $\alpha \in (0,1]$ is the coefficient for the exploited class of biased compressor $\mathcal{B}(\alpha) = \{\mathcal{C}:\mathbb{R}^d \to \mathbb{R}^d \,|\, \mathbb{E} [ \|C(x) - x\|^2 ] \le (1 - \alpha)\|x\|^2, \forall x \in \mathbb{R}^d \}$ by the $n$ clients. The \texttt{TopK} compressor returns sparse vectors filled with zeros, except $k$ position, which corresponds to $k$ maximum values in absolute value and which are unchanged by the compressor. Even if this compressor breaks ties arbitrarily, it is possible to show that $\alpha = \frac{k}{d}$. In general, the coefficient $\alpha$ is compressor dependent. This parameter is defined without considering properties of $f_i$. The quantities $\beta, \theta, \beta/\theta$ are derived from $\alpha$; consequently, they do not depend on $L_{f_i}$.
	
	The quantity $\tilde{L} \eqdef \left(\frac{1}{n} \sum L_i ^2\right)^{1/2}$ from standard \algname{EF21} analysis, as we saw with special consideration in fact, is improvable. This improved version of \algname{EF21-W} allows to make $\tilde{L}'(w) \eqdef \left(\frac{1}{n} \sum L_i ^2 / w_i \right)^{1/2}$ with $w_i \eqdef \frac{N_i}{N}$. Here $N_i$ is the number of virtual workers (clones of client number $i$) and $N=\sum_{i=1}^{n} N_i$. Minimum possible $\tilde{L}$ as a function of $N_i/N$ under assumption that $N_i/N$ is real number is equal to:
	\begin{eqnarray}
		\label{frm:improved_L_tilda}
		\tilde{L}' \eqdef \dfrac{1}{n} \sum L_i
	\end{eqnarray}
	
	It's always the case that $\tilde{L}^2 \ge 
	\tilde{L}'^2$ because $\tilde{L}^2 - \tilde{L}'^2 = \mathrm{Var}_{i \sim \mathrm{u.a.r.} [n]} [L_i] \ge 0$.
	Because $x^2$ is monotonically increasing on $\{ x \in \mathbb{R}:x \ge 0 \}$, we can conclude that it is always the case that $\tilde{L} \ge \tilde{L}'$. The difference $\tilde{L} - \tilde{L}'$ has the following upper bound: 
	\begin{eqnarray*}
		\label{frm:improved_L_tilda_diff}
		\tilde{L} - \tilde{L}' = \sqrt{(\tilde{L} - \tilde{L}')^2} = \sqrt{\tilde{L}^2 + \tilde{L}'^2 - 2\tilde{L} \cdot \tilde{L}'} = \\
		\sqrt{\tilde{L}^2 + \tilde{L}'(\tilde{L}' - 2\tilde{L})}  \le \\
		\sqrt{\tilde{L}^2 + \tilde{L}'(\tilde{L}' - 2\tilde{L}')} = \\		
		\sqrt{\dfrac{1}{n} \sum_{i=1}^{n} L_i^2 + \left(\dfrac{1}{n} \sum_{i=1}^{n} L_i\right) ^2 - 2 \cdot \left(\dfrac{1}{n} \sum_{i=1}^{n} L_i\right) ^2}
		= \sqrt{\dfrac{1}{n} \sum_{i=1}^{n} \left(L_i - \dfrac{1}{n} \sum_{i=1}^{n} L_i\right) ^2} \ge 0
	\end{eqnarray*}
	
	Next, we can observe that the following equality for $\tilde{L} - \tilde{L}'$ holds:
	\begin{eqnarray*}
		\tilde{L} - \tilde{L}' =  (\tilde{L} - \tilde{L}')\left(\frac{\tilde{L} + \tilde{L}'}{\tilde{L} + \tilde{L}'}\right) = \frac{\tilde{L}^2 - \tilde{L}'^2}{\tilde{L} + \tilde{L}'} = \frac{1}{\tilde{L} + \tilde{L}'} \cdot {\dfrac{1}{n} \sum_{i=1}^{n} \left(L_i - \dfrac{1}{n} \sum_{i=1}^{n} L_i\right) ^2} \\
		\tilde{L} - \tilde{L}' \propto {\dfrac{1}{n} \sum_{i=1}^{n} \left(L_i - \dfrac{1}{n} \sum_{i=1}^{n} L_i\right) ^2}
	\end{eqnarray*}
	
	Hidden coefficient of proportion is equal to $\dfrac{1}{\tilde{L}+\tilde{L}'} \le \dfrac{1}{2\tilde{L}'}=\dfrac{1}{2} \cdot \dfrac{1}{\tilde{L}'}$. As a consequence, difference $\tilde{L} - \tilde{L}'$ (if ignore factor $1/2$) is bound by the estimated variance of $L_i$ divided by the mean of $L_i$, also known as \textit{index of dispersion} in statistics. 

	From this consideration, we can observe that \algname{EF-21VC} have arbitrarily better step size as the variance of $L_i$ is increasing faster than $\frac{2}{(\tilde{L}+\tilde{L}')/2}$. The synthetic experiments empirically study the behaviour of \algname{EF21} and \algname{EF21-W} during varying quantity $\mathrm{Var}_{i \sim \mathrm{u.a.r.} [n]} [L_i]$. 
	
	Finally let us remind that for a finite sum structure $f(x) = \frac{1}{n} \sum_{i=1}^{n} f_i(x)$ the following theoretical bounds hold: $L_f \le \frac{1}{n} \sum_{i=1}^{n} L_i \le \max L_{f_i} \le n \cdot L_f$, which are usefull for sanity checks of experiment results.
	
	\subsection{Role of Our Improvement for EF21}
	We want to highlight that our improvement has important consequences. The parameter $\tilde{L}'$ during computing step size is multiplied by factor $\sqrt{\frac{\beta}{\theta}}$. Even for situations when $\tilde{L}'$ is only a bit smaller compared to $\tilde{L}$, but for computing theoretical step size, the $\tilde{L}'$ is multiplied by factor $\sqrt{\frac{\beta}{\theta}}$. It turns out that factor $\sqrt{\frac{\beta}{\theta}}$ can be arbitrarily big as $d$ increases. We demonstrated this in Fig. \ref{fig:beta_over_theta_theoretical}). If $d$ is increasing and parameter $k$ of \algname{TopK} compressor is fixed, then even a small improvement in $\tilde{L}'$ dramatically improves step size.
	
	%\begin{wrapfigure}{r}{0.1\textwidth}
	%\begin{figure*}
	%	\begin{minipage}[b]{\textwidth}
	%		\centering
	%		\includegraphics[width=\textwidth]{./ef21-vc-figs/ef21vc-compressors-as-function-of-d}
	%		\captionof{figure}{Factor $\sqrt{{\beta}/{\theta}}$ as a function of optimization variable dimension $d$ which plays a role during computing step-size for \algname{EF21-W} $\gamma = ( L + \tilde{L} \sqrt{{\beta}/{\theta}})$
	%		}
	%		\label{fig:beta_over_theta_theoretical}
	%	\end{minipage}
	%	\caption*{}
	%\end{figure*}
	%\end{wrapfigure}	
	
	\begin{center}	
		\begin{figure*}[t]
			\centering
			\captionsetup[sub]{font=normalsize,labelfont={}}	
			\captionsetup[subfigure]{labelformat=empty}		

			\begin{subfigure}[ht]{1.0\textwidth}
				\includegraphics[width=\textwidth]{./ef21-vc-figs/ef21vc-compressors-as-function-of-d.pdf} \caption{}
			\end{subfigure}
			
			%\vspave{-1pt}
			\caption{Factor $\sqrt{{\beta}/{\theta}}$ as a function of optimization variable dimension $d$ which plays a role during computing step-size for \algname{EF21-W} $\gamma = ( L + \tilde{L} \sqrt{{\beta}/{\theta}})$}
			\label{fig:beta_over_theta_theoretical}
		\end{figure*}
	\end{center}

	\subsection{Computing and Software environment} We used the Python software suite \texttt{FL\_PyTorch} \cite{burlachenko2021fl_pytorch} to simulate the distributed environment for training. We carried out experiments on a compute node with \texttt{Ubuntu 18.04 LTS}, $256$ GBytes of DRAM DDR4 memory at $2.9$GHz, and $48$ cores ($2$ sockets with $24$ cores per socket) of \texttt{Intel(R) Xeon(R) Gold 6246 CPU at $3.3$GHz}. We used double-precision arithmetic during computing gradient oracles. Computations were carried in \texttt{CPU}.
	
	\subsection{Synthetic Experiments}
	\label{sec:syn_experiments}
	
	\subsubsection{Problem}
	In our synthetic experiments, we consider the minimization of the function:
	\begin{equation*}
		\min \limits_{x \in \mathbb{R}^d} \left\{f(x) = \frac{1}{n}\sum \limits_{i=1}^n f_i(x)\right\}.
	\end{equation*}
	
	In our \textit{first synthetic experiment} we consider the case, when $f_i(x)$ are strongly convex:
	\begin{gather*}
		f_i(x) \eqdef \dfrac{1}{n_i} \norm{\bA_i x - {b_i}}^2 + \frac{\alpha}{2} \|x\|^2
	\end{gather*}
	In this case it can be shown that $L_{f_i} = \dfrac{2}{n_i} \lambda_{\max}({A_i}^\top A_i) + \alpha$.
	
	In our \textit{second synthetic experiment} we consider the case, when $f_i(x)$ are non-convex:
	\begin{gather*}
		f_i(x) \eqdef \dfrac{1}{n_i} \norm{\bA_i x - {b_i}}^2 + \alpha \cdot \sum_{j=1}^{d} \dfrac{x_j^2}{x_j^2 + 1}
	\end{gather*}
	
	
	
	It can be shown that $L_{f_i} = \dfrac{2}{n_i} \lambda_{\max}({A_i}^\top A_i) + 2 \alpha$. 
	The regularizer $r(x) = \sum_{j=1}^{d} \dfrac{x_j^2}{x_j^2 + 1}$ has the spectrum $\lambda_j \left( \nabla^2 r(x) \right) \in [-\frac{1}{2}, 2], \forall j \in [d]$. To guarantee that function $f_i(x)$ is non-convex the following bound should holds:
	$$ \dfrac{2}{n_i} \lambda_{\min}({A_i}^\top A_i) - \frac{1}{2} \alpha \le 0 \implies \alpha \ge  \lambda_{\min}\left(\dfrac{4}{n_i} \cdot {A_i}^\top A_i\right).$$
	
	
	\subsubsection{Datasets Generation}
	
	First, we assume that the user provides two parameters $\mu \in \mathbb{R}_+$ and $L \in \mathbb{R}_+$. These parameters define the construction of strongly convex function $f_i(x)$, which are modified by meta-parameters $q \in [-1,1], z > 0$ described next.
	
	\paragraph{First Step.} Each client has
	$f_i(x) \eqdef \dfrac{1}{n_i} \norm{\bA_i x - {b_i}}^2$ where $A_i$ is initialized in such way that $f_i$ is $L_{f_i}$ smooth and $\mu_{f_i}$ strongly convex. Parameters are defined in the following way: 
	\[L_{f_i}=\dfrac{i}{n} \cdot (L-\mu) + \mu, \mu_{f_i} = \mu.\]
	
	\paragraph{Second Step.}
	We introduce scalar value $q \in [-1,+1]$, which informally plays the role of meta parameter to change the distribution of $L_{f_i}$ and make values of $L_{f_i}$ close to one of the following: (i) $\mu$; (ii) $L$; (iii) $(L+\mu)/2$. 
	
	The exact modification of $L_{f_i}$ depends on the sign of meta parameter $q$.
	
	\paragraph{Case $q \in [0,1]$.} In this case for first $n/2$ (i.e. $i \in [0, n/2]$) compute the value $L_{f_i,q} = \mathrm{lerp}(L_{f_i}, \mu, q)$, where $\mathrm{lerp}(a,b,t):\RD \times \RD \times [0,1] \to \RD$ is linear interpolation:	
	\[
	\mathrm{lerp}(a, b, t) = a (1-t) + bt.
	\]
	
	The last $n/2$ ($i \in [n/2+1, n]$) compute the value $L_{f_i,q} = \mathrm{lerp}(L_{f_i}, L, q)$. For example, if $q=0$ then $L_{f_i,q}=L_{f_i}, \forall i \in [n]$, and if $q=1$ then $L_{f_i,q} = \mu$ for first ${n}/{2}$ clients and $L_{f_i,q} = L$ for last ${n}/{2}$ clients.
	
	
	\paragraph{Case $q \in [-1,0]$.} In this for all $n$ clients the new value $L_{f_i,q} = \mathrm{lerp}(L_{f_i}, ({L+\mu})/{2}, -q)$. In this case for example if $q=0$ then $L_{f_i,q}=L_{f_i}$ and if $q=-1$ then $L_{f_i,q} = ({L+\mu})/{2}$.
	
	Essentially the process firstly fills the $A_i$ in such form that essentially $L_{f_i}$ forms a uniform spectrum in $[\mu, L]$ with the center of this spectrum equal to $a=\frac{L+\mu}{2}$. And then as $q \to 1$, the variance of $L_{f_i,q}$ is increasing.
	
	\paragraph{Third Step.} We use these new values  $L_{f_i,q}$ for all $i \in [n]$ clients as a final target $L_{f_i}^{\mathrm{new}}$ values. Due to numerical issues, we found that it's worthwhile for the first and last client to add extra scaling. First client scales $L_{f_1,q}$ by 
	factor $1/z$, and last $n$-th client scales $L_{f_n,q}$ by factor $z$. Here $z \ge 0$ is an additional meta-parameter.
	
	\paragraph{Fourth Step.} Next obtained values are used to generate $A_i$ in such way that $\nabla^2 f_i(x)$ has uniform spectrum in $[\mu_{f_i,q,z}, L_{f_i,q,z}]$.
	
	\paragraph{Fifth Step.} As a last step the objective function $f(x)$ is scaled in such a way that it is $L$ smooth with constant value $L$. The $b_i$ for each client is initialized as $b_i \eqdef A_i \cdot x_{\mathrm{solution}}$, where $x_{\mathrm{solution}}$ is fixed solution.
	
	This process induces variance on $L_i$ as a function of $(q,z)$.
	
	\subsubsection{Experimental Setup}
	
	In synthetic experiments, we have used the maximum allowable step size suggested by the theory of \algname{EF21} and for the proposed \algname{EF21-W} algorithms. The initial shift for gradient estimators has been initialized as $g_i^0 = \nabla f_i (x^0)$. The number of clients in simulation $n=2000$, dimension of optimization problem $d=10$, number of samples per client $n_i=10$, and number of communication rounds is $r=10\,000$. For both \algname{EF21} and \algname{EF21-W} clients use \algname{TopK[K=1]} biased contractive compressor. We present optimization problem instances with different relationships between $\tilde{L}$ and $\tilde{L}'$. Because  $\tilde{L}'$ is equal to the arithmetic mean of $L_i$, it is always better(not bigger) compared to $\tilde{L}$ defined as the quadratic mean of $L_i$.
	
	\subsubsection{Experimental Results for Strongly Convex Case.}
	\begin{center}	
		\begin{figure*}[t]
			\centering
			\captionsetup[sub]{font=normalsize,labelfont={}}	
			\captionsetup[subfigure]{labelformat=empty}
			%\captionsetup{position=top}
			
			\begin{subfigure}[ht]{0.44\textwidth}
				\includegraphics[width=\textwidth]{./ef21-vc-figs/expsyn/ef21-vc-run-33-gradsqr.pdf} \caption{ (a) $q=1,z=10^4$ }
			\end{subfigure}		
			\begin{subfigure}[ht]{0.44\textwidth}
				\includegraphics[width=\textwidth]{./ef21-vc-figs/expsyn/ef21-vc-run-34-gradsqr.pdf} \caption{ (b) $q=1,z=10^3$ }
			\end{subfigure}
			
			\begin{subfigure}[ht]{0.44\textwidth}
				\includegraphics[width=\textwidth]{./ef21-vc-figs/expsyn/ef21-vc-run-18-gradsqr.pdf} \caption{ (c) $q=1,z=10^2$}
			\end{subfigure}		
			\begin{subfigure}[ht]{0.44\textwidth}
				\includegraphics[width=\textwidth]{./ef21-vc-figs/expsyn/ef21-vc-run-22-gradsqr.pdf} \caption{ (d) $q=0.8,z=1$}
			\end{subfigure}
			
			%\vspave{-1pt}
			\caption{\algname{EF21} and \algname{EF21-W} for convex smooth optimization with \algname{TopK[K=1]} client compressor, $n=2\,000$, $d=10$. Regularization term $\alpha \cdot \frac{\|x\|^2}{2}$, $\alpha=0.01$. The step sizes used are theoretical. The characteristic of each problem is presented in Table \ref{tbl:exp_syn_der_quantities}.}
			\label{fig:syn_ef21_vc}
		\end{figure*}
	\end{center}
	
	The result of experiments for training linear regression model with a convex regularizer is presented in Figure \ref{fig:syn_ef21_vc}. The regularization term $\phi(x) \eqdef \frac{\alpha}{2} \|x\|^2$, and $\alpha=0.01$. Instances of optimization problems were generated for values $L=50, \mu = 1$ with several values of $q,z$. The summary of derived quantities is presented in Table \ref{tbl:exp_syn_der_quantities}. We present several optimization problems to demonstrate the possible different relationships between $\tilde{L}$ and $\tilde{L}'$. As we see from experiments, the \algname{EF21-W} is superior as the variance of $L_{f_i}$ tends to increase. The plots in Figure \ref{fig:syn_ef21_vc} (a) -- (d) correspond to decreasing variance of $L_{f_i}$. As we see, as the variance of $L_i$ decreases, the difference between \algname{EF21-W} and \algname{EF21} also tends to decrease. However, \algname{EF21-W} is always at least as best as \algname{EF21}.

	The number of rounds for simulation is $r=10\,000$. During each round, each client sends one scalar in \texttt{FP64} and requires $64$ bits of a payload while sending through a communication channel. Sending information from clients to master during $10$K rounds requires $6.4\cdot10^5$ bits of uplink traffic per client for transferring values. In practice, when using \algname{TopK}, it is necessary to send information about indices.

	\begin{table}[h]
		\begin{center}
			\caption{Summary of derived quantities which defines theoretical step size strongly for convex optimization experiments in Figure \ref{fig:syn_ef21_vc}.}
			\label{tbl:exp_syn_der_quantities}
			\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|}
				\hline
				Tag & $L_f$ & $q$ & $z$ & $\mathrm{Var}[L_i]$ & $\sqrt{\frac{\beta}{\theta}}$ & $\tilde{L}$ & $\tilde{L}'$ & $\gamma_{\mathrm{ef21}}$ & $\gamma_{\mathrm{ef21-vc}}$ \\
				\hline
				(a) & $50$ & $1$ & $10^4$ & $4.45 \cdot 10^6$ & $18.486$ & $2111.90$ & $52.04$ & $2.55\cdot10^{-5}$ & $9.87 \cdot 10^{-4}$ \\
				\hline
				(b) & $50$ & $1$ & $10^3$ & $1.97 \cdot 10^6$ & $18.486$ & $1408.49$ & $63.56$ & $3.83\cdot10^{-5}$ & $8.16 \cdot 10^{-4}$ \\
				\hline
				(c) & $50$ & $1$ & $10^2$ & $1.08 \cdot 10^5$ & $18.486$ & $339.34$ & $80.97$ & $1.58\cdot10^{-4}$ & $6.46 \cdot 10^{-4}$ \\
				\hline
				(d) & $50$ & $0.8$ & $1$ & $5.42 \cdot 10^3$ & $18.486$ & $112.51$ & $85.03$ & $4.69\cdot10^{-4}$ & $6.16 \cdot 10^{-4}$\\
				\hline
			\end{tabular}
		\end{center}
	\end{table}
	
	
	\subsubsection{Experimental Results for Non-Convex Case.}
	\begin{center}	
		\begin{figure*}[t]
			\centering
			\captionsetup[sub]{font=normalsize,labelfont={}}	
			\captionsetup[subfigure]{labelformat=empty}
			%\captionsetup{position=top}
			
			\begin{subfigure}[ht]{0.44\textwidth}
				\includegraphics[width=\textwidth]{./ef21-vc-figs/expsyn/ef21-vc-run-33-gradsqr-ncvx.pdf} \caption{ (a) $q=1,z=10^4$ }
			\end{subfigure}		
			\begin{subfigure}[ht]{0.44\textwidth}
				\includegraphics[width=\textwidth]{./ef21-vc-figs/expsyn/ef21-vc-run-34-gradsqr-ncvx.pdf} \caption{ (b) $q=1,z=10^3$ }
			\end{subfigure}
			
			\begin{subfigure}[ht]{0.44\textwidth}
				\includegraphics[width=\textwidth]{./ef21-vc-figs/expsyn/ef21-vc-run-18-gradsqr-ncvx.pdf} \caption{ (c) $q=1,z=10^2$}
			\end{subfigure}		
			\begin{subfigure}[ht]{0.44\textwidth}
				\includegraphics[width=\textwidth]{./ef21-vc-figs/expsyn/ef21-vc-run-22-gradsqr-ncvx.pdf} \caption{ (d) $q=0.8,z=1$}
			\end{subfigure}
			
			%\vspave{-1pt}
			\caption{Comparison of the performance of standard \algname{EF21} and \algname{EF21-W} for non-convex smooth optimization. The used compressor is \algname{TopK[K=1]}. The number of clients $n=2\,000$. The regularization coefficient for non-convex regularizes $\lambda=100$. The used step size is theoretical. The characteristic of each problem is presented in Table \ref{tbl:exp_syn_der_quantities_noncvx}.}
			\label{fig:syn_ef21_vc_noncvx}
		\end{figure*}
	\end{center}
	
	The result of experiments for training linear regression model with a non-convex regularizer is presented in Figure \ref{fig:syn_ef21_vc_noncvx}. The regularization coefficient $\alpha$ for regularization term in a form of of $\alpha \cdot \sum_{j=1}^{d} \dfrac{x_j^2}{x_j^2 + 1}$ is equal $\alpha=100$. Instances of optimization problems were generated for values $L=50, \mu = 1$ and several values of $q,z$. The summary of derived quantities is presented in Table \ref{tbl:exp_syn_der_quantities_noncvx}.  We present various instances of optimization problems to demonstrate the different relationships between $\tilde{L}$ and $\tilde{L}'$. As we see in the case of small variance of $L_{f_i}$ is at least as best as standard \algname{EF21}. The number of rounds for simulation is $r=10\,000$. Each client sends one scalar in \texttt{FP64} during each round. It requires $64$ bits of a payload while sending through a communication channel without considering the actual index.
	
	\begin{table}[h]
		\begin{center}
			\caption{Summary of derived quantities which defines theoretical step size for non-convex optimization experiments in Figure \ref{fig:syn_ef21_vc_noncvx}.}
			\label{tbl:exp_syn_der_quantities_noncvx}
			\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|}
				\hline
				Tag & $L_f$ & $q$ & $z$ & $\mathrm{Var}[L_i]$ & $\sqrt{\frac{\beta}{\theta}}$ & $\tilde{L}$ & $\tilde{L}'$ & $\gamma_{\mathrm{ef21}}$ & $\gamma_{\mathrm{ef21-vc}}$ \\
				\hline
				(a) & $50$ & $1$ & $10^4$ & $4.45 \cdot 10^6$ & $18.486$ & $2126.25$ & $252.035$ & $2.52\cdot10^{-5}$ & $2.03 \cdot 10^{-4}$ \\
				\hline
				(b) & $50$ & $1$ & $10^3$ & $1.97 \cdot 10^6$ & $18.486$ & $1431.53$ & $263.55$ & $3.74\cdot10^{-5}$ & $1.95 \cdot 10^{-4}$ \\
				\hline
				(c) & $50$ & $1$ & $10^2$ & $1.08 \cdot 10^5$ & $18.486$ & $433.05$ & $280.958$ & $1.21\cdot10^{-4}$ & $1.83 \cdot 10^{-4}$ \\
				\hline
				(d) & $50$ & $0.8$ & $1$ & $5.42 \cdot 10^3$ & $18.486$ & $294.39$ & $285.022$ & $1.17\cdot10^{-4}$ & $1.81 \cdot 10^{-4}$\\
				\hline
			\end{tabular}
		\end{center}
	\end{table}
	
	\subsection{Experiments on Real Datasets}
	
	In this section, we provide additional numerical experiments in which we compare \algname{EF21} and \algname{EF21-W}. We address the problem of training a binary classifier via a logistic model on several \texttt{LIBSVM} datasets \cite{chang2011libsvm} with non-convex regularization.
	
	\paragraph{Experiment setup.}
	We conducted distributed training of a logistic regression model on \texttt{W1A}, \texttt{W2A}, \texttt{W3A}, \texttt{PHISHING}, \texttt{MUSHROOMS}, \texttt{AUSTRALIAN} datasets with non-convex regularization. For all datasets, we consider the minimization of the following function $f(x)$:
	\begin{gather*}
		f(x) = \dfrac{1}{n} \sum_{i=1}^{n} f_i(x), \\
		f_i(x) \eqdef \dfrac{1}{n_i} \sum_{j=1}^{n_i} \log \left(1+\exp({-y_{ij} \cdot a_{ij}^{\top} x})\right) + \lambda \cdot \sum_{j=1}^{d} \dfrac{x_j^2}{x_j^2 + 1},\\
		(a_{ij},  y_{ij}) \in \mathbb{R}^{d} \times \{-1,1\}.
	\end{gather*}
	
	The initial shifts for \algname{EF21} are $g_i^0 = \nabla f_i(x^0), \forall i \in [n]$. For algorithm \algname{EF21} and \algname{EF21-W} comparison, we used the largest step size allowed by theory. The term $\phi(x)$ is a non-convex regularizer, with eigenvalues in the set $\left[-\frac{1}{2}, 2\right]$. We use the dataset shuffling algorithm described in Section \ref{app:dataset_shuffling_for_libsvm}.
	
	\subsubsection{Dataset Shuffling Strategy}
	\label{app:dataset_shuffling_for_libsvm}
	Our dataset shuffling strategy heuristically splits data points so that $\texttt{Var}[L_i]$ is maximized. It consists of the following steps:
	
	\paragraph{1. Sort Datapoints from Dataset according to L-smooth constant.} Sort all data points according to the smooth constant of the loss function for each data point.
	
	\paragraph{2. Assign One single Datapoint for each client} Assume that there are total $m$ datapoints in the dataset, and the total number of clients is $n$. At the beginning each client $i$ holds a single datapoint $\lfloor (i-1 + 1/2) \cdot \frac{m}{n}\rfloor$.
	
	\paragraph{3. Pass-Through All Points.} Initialize set $F=\{\}$. Next, we pass through all points except those assigned from the previous step. For each point we find the best client $i'\in [n] \backslash F$ to assign the point in a way that assignment of point to client $i'$ maximize $\mathrm{Var}[L_{f_i}] = \frac{1}{n} \sum_{i=1}^{n} L_{f_i}^2 - (\frac{1}{n} \sum_{i=1}^{n} L_{f_i})^2$. Once the client already has $\lceil \frac{m}{n} \rceil$ data points assigned to it, the client is added to the set $F$.
	
	The set $F$ in the last step guarantees each client will have $\frac{m}{n}$ data points. In general, this is a heuristic greedy strategy that approximately maximizes $\mathrm{Var}[L_{f_i}]$ under the constraint that each client has the same amount of data points equal to $\lfloor \frac{m}{n} \rfloor$. Due to its heuristic nature, the Algorithm does not provide deep guarantees, but it was good enough for our experiments. The complexity of Algorithms is $\mathcal{O}(nm \cdot C)$, where $C$ is cost of computing $L_{f_i}$ where $f_i:\mathbb{R}^d \to \mathbb{R}$ has $\lfloor \frac{m}{n} \rfloor$ datapoints.
		
	\begin{center}	
		\begin{figure*}[t]
			\centering
			\captionsetup[sub]{font=normalsize,labelfont={}}	
			\captionsetup[subfigure]{labelformat=empty}
			%\captionsetup{position=top}
			
			\begin{subfigure}[ht]{0.32\textwidth}
				\includegraphics[width=\textwidth]{./ef21-vc-figs/expreal/fig1-09JULY23-w1a.pdf} \caption{ (a) \texttt{W1A}, $d=302$ }
			\end{subfigure}		
			\begin{subfigure}[ht]{0.32\textwidth}
				\includegraphics[width=\textwidth]{./ef21-vc-figs/expreal/fig2-09JULY23-w2a.pdf} \caption{ (b) \texttt{W2A}, $d=302$ }
			\end{subfigure}
			\begin{subfigure}[ht]{0.32\textwidth}
				\includegraphics[width=\textwidth]{./ef21-vc-figs/expreal/fig3-09JULY23-w3a.pdf} \caption{ (c) \texttt{W3A}, $d=302$ }
			\end{subfigure}
			
			\begin{subfigure}[ht]{0.32\textwidth}
				\includegraphics[width=\textwidth]{./ef21-vc-figs/expreal/fig4-09JULY23-mushrooms} \caption{ (d) \texttt{MUSHROOMS}, $d=114$ }
			\end{subfigure}
			\begin{subfigure}[ht]{0.32\textwidth}
				\includegraphics[width=\textwidth]{./ef21-vc-figs/expreal/fig5-09JULY23-splice.pdf} \caption{ (e) \texttt{SPLICE}, $d=62$ }
			\end{subfigure}
			\begin{subfigure}[ht]{0.32\textwidth}
				\includegraphics[width=\textwidth]{./ef21-vc-figs/expreal/fig6-09JULY23-phishing.pdf} \caption{ (f) \texttt{PHISHING}, $d=70$ }
			\end{subfigure}
			
			%\vspave{-1pt}
			\caption{Comparison of the performance of standard \algname{EF21} and \algname{EF21-W} for non-convex Logistic Regression. The used compressor is \algname{TopK[K=1]}. The number of clients $n=1\,000$. Regularization coefficient $\lambda=0.001$. The step size used is theoretical. Extra characteristics are in Table \ref{tbl:exp_real_der_quantities}.}
			\label{fig:real_ef21_vc_ncvx}
		\end{figure*}
	\end{center}
	
	
	
	\begin{center}	
		\begin{figure*}[t]
			\centering
			\captionsetup[sub]{font=normalsize,labelfont={}}	
			\captionsetup[subfigure]{labelformat=empty}
			%\captionsetup{position=top}
			
			\begin{subfigure}[ht]{0.50\textwidth}
				\includegraphics[width=\textwidth]{./ef21-vc-figs/expreal/fig7-10JULY23-australian} \caption{ \texttt{AUSTRALIAN}, $d=16$ }
			\end{subfigure}
			
			%\vspave{-1pt}
			\caption{Comparison of the performance of standard \algname{EF21} and \algname{EF21-W} for non-convex Logistic Regression. The used compressor is \algname{TopK[K=1]}. The number of clients $n=200$. Regularization coefficient $\lambda=1000$. The used step size is theoretical. Extra characteristics are in Table \ref{tbl:exp_real_der_quantities}.}
			\label{fig:real_ef21_vc_ncvx_australian}
		\end{figure*}
	\end{center}

	\begin{table}[h]
		\begin{center}
			\caption{Summary of derived quantities which defines theoretical step size for non-convex optimization experiments in Figure \ref{fig:real_ef21_vc_ncvx}.}
			\label{tbl:exp_real_der_quantities}
			\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|}
				\hline
				Tag & $L_f$ & $\mathrm{Var}[L_i]$ & $\sqrt{\frac{\beta}{\theta}}$ & $\tilde{L}$ & $\tilde{L}'$ & $\gamma_{\mathrm{ef21}}$ & $\gamma_{\mathrm{ef21-vc}}$ \\
				\hline
				\tiny{(a) W1A} & $0.781$ & $3.283$ & $602.49$ & $2.921$ & $2.291$ & $5.678\cdot10^{-4}$ & $7.237 \cdot 10^{-4}$ \\
				\hline
				\tiny{(b) W2A} & $0.784$ & $2.041$ & $602.49$ & $2.402$ & $1.931$ & $6.905\cdot10^{-4}$ & $8.589\cdot10^{-4}$ \\
				\hline
				\tiny{(c) W3A} & $0.801$ & $1.579$ & $602.49$ & $2.147$ & $1.741$ & $7.772\cdot10^{-4}$ & $9.523 \cdot 10^{-4}$ \\
				\hline
				\tiny{(d) MUSHROOMS} & $2.913$ & $0.505$ & $226.498$ & $3.771$ & $3.704$ & $1.166\cdot10^{-3}$ & $1.187\cdot10^{-3}$\\
				\hline
				\tiny{(e) SPLICE} & $96.082$ & $223.094$ & $122.497$ & $114.43$ & $113.45$ & $7.084\cdot10^{-5}$ & $7.14\cdot10^{-5}$\\
				\hline
				\tiny{(f) PHISHING} & $0.412$ & $9.2 \cdot 10^{-4}$ & $138.498$ & $0.429$ & $0.428$ & $1.670\cdot10^{-2}$ & $1.674 \cdot 10^{-2}$\\			
				\hline				
				\tiny{(g) AUSTRALIAN} & $3.96 \cdot 10^6 $ & $1.1 \cdot 10^{16}$ & $18.486$ & $3.35 \cdot 10^{7}$ & $3.96 \cdot 10^{6}$ & $9.733\cdot10^{-10}$ & $8.007 \cdot 10^{-9}$\\
				\hline				
			\end{tabular}
		\end{center}
	\end{table}
	
	\subsubsection{Result of Training Non-Convex Logistic Regression Model}
	The results are presented in Figure \ref{fig:real_ef21_vc_ncvx} and Figure \ref{fig:real_ef21_vc_ncvx_australian}. The important quantities for these instances of optimization problems are summarized in Table \ref{tbl:exp_syn_der_quantities_noncvx}.
	
	From Figures \ref{fig:real_ef21_vc_ncvx} (a), (b), (c), we can observe that for these datasets, the \algname{EF21-W} is better, and this effect is observable in practice and is not negligible. For example, from these examples, we can observe that $12.5$K rounds of \algname{EF21-W} corresponds to only $10$K rounds of \algname{EF21}. This improvement is essential for Federated Learning, in which communication rounds and communicated information are the main bottlenecks. Figures \ref{fig:real_ef21_vc_ncvx} (d), (e), (f) demonstrate that sometimes the \algname{EF21-W} can have practical behavior close to \algname{EF21}, even if there is an improvement in step-size (For exact values of step size see Table \ref{tbl:exp_syn_der_quantities_noncvx}).
	
	The experiment on \texttt{AUSTRALIAN} datasets are presented in Figure \ref{fig:real_ef21_vc_ncvx_australian}. This example demonstrates that in this \texttt{LIBSVM} benchmark datasets, the relative improvement in the number of rounds for \algname{EF21-W} compared to \algname{EF21} is considerable. For example $40$K rounds of \algname{EF21} corresponds to $5$K rounds of \algname{EF21-W} in terms of attainable $\| \nabla f(x^k)\|^2$.
	
	%=========================================================================
	%\clearpage
	%\section{References}
	%\printbibliography[heading=none]	
	%=========================================================================
%\end{document}

